Symbolic vs. Bounded Synthesis for Petri Games

Petri games are a multiplayer game model for the automatic synthesis of distributed systems. We compare two fundamentally different approaches for solving Petri games. The symbolic approach decides the existence of a winning strategy via a reduction to a two-player game over a finite graph, which in turn is solved by a fixed point iteration based on binary decision diagrams (BDDs). The bounded synthesis approach encodes the existence of a winning strategy, up to a given bound on the size of the strategy, as a quantified Boolean formula (QBF). In this paper, we report on initial experience with a prototype implementation of the bounded synthesis approach. We compare bounded synthesis to the existing implementation of the symbolic approach in the synthesis tool ADAM. We present experimental results on a collection of benchmarks, including one new benchmark family, modeling manufacturing and workflow scenarios with multiple concurrent processes.

==> eptcsdata.tex <==
\providecommand{\firstpage}{23}
\providecommand{\publicationstatus}{D. Fisman, S. Jacobs (Eds.): Sixth Workshop on Synthesis (SYNT 2017)\\
EPTCS 260, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.260.5}{10.4204/EPTCS.260.5}}
\pdfoutput=1

